Semi-supervised novelty detection using ensembles with regularized disagreement

Deep neural networks often predict samples with high confidence even when they come from unseen classes and should instead be flagged for expert evaluation. Current novelty detection algorithms cannot reliably identify such near OOD points unless they have access to labeled data that is similar to these novel samples. In this paper, we develop a new ensemble-based procedure for semi-supervised novelty detection (SSND) that successfully leverages a mixture of unlabeled ID and novel-class samples to achieve good detection performance. In particular, we show how to achieve disagreement only on OOD data using early stopping regularization. While we prove this fact for a simple data distribution, our extensive experiments suggest that it holds true for more complex scenarios: our approach significantly outperforms state-of-the-art SSND methods on standard image data sets (SVHN/CIFAR-10/CIFAR-100) and medical image data sets with only a negligible increase in computation cost.

==> tables/binary_classifier.tex <==
\hyphenpenalty10000
\begin{tabularx}{0.7\textwidth}{ll| c}
\toprule
\makecell{ID data} & \makecell{OOD data} & \makecell{Binary classifier} \\
& & \multicolumn{1}{c}{AUROC $\uparrow$} \\
\midrule
$\text{ SVHN }$ & $\text{ CIFAR10 }$ & 0.99 \\
$\text{ CIFAR10 }$ & $\text{ SVHN }$ & 1.00 \\
$\text{ CIFAR100 }$ & $\text{ SVHN }$ & 1.00 \\
\midrule
$\text{ SVHN[0:4] }$ & $\text{ SVHN[5:9] }$ & 0.82 \\
$\text{ CIFAR10[0:4] }$ & $\text{ CIFAR10[5:9] }$ & 0.83 \\
$\text{ CIFAR100[0:49] }$ & $\text{ CIFAR100[50:99] }$ & 0.61 \\

\midrule
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 2 (A) }$ & 0.94 \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 2 (W) }$ & 0.51 \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 5 (A) }$ & 1.00 \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 5 (W) }$ & 1.00 \\
\midrule
$\text{ CIFAR100 }$ & $\text{ CIFAR100-C sev 2 (A) }$ & 0.83 \\
$\text{ CIFAR100 }$ & $\text{ CIFAR100-C sev 2 (W) }$ & 0.50 \\
$\text{ CIFAR100 }$ & $\text{ CIFAR100-C sev 5 (A) }$ & 1.00 \\
$\text{ CIFAR100 }$ & $\text{ CIFAR100-C sev 5 (W) }$ & 1.00 \\

\midrule
$\text{ Tiny ImageNet }$ & $\text{ Tiny ObjectNet }$ & 1.00 \\

\midrule
\multicolumn{2}{c|}{Average} & 0.94 \\

\bottomrule
\end{tabularx}

==> tables/imagenet.tex <==
\setlength{\tabcolsep}{1pt}
\hyphenpenalty10000
\begin{tabularx}{\textwidth}{@{}ll @{}| @{\hskip 0.2cm} X X X X X X X X X  @{}}
\toprule
\makecell[l]{ ID data } & \makecell[l]{ OOD data } & \makecell[l]{ kNN } & \makecell[l]{ Vanilla\\Ensembles } & \makecell[l]{ OE } & \makecell[l]{ Mahal. } & \makecell[l]{ DPN } & \makecell[l]{ Mahal-T } & \makecell[l]{ MCD } & \makecell[l]{ RETO\\(rand init) } & \makecell[l]{ RETO\\(pretrained) } \\
& & \multicolumn{9}{c}{AUROC $\uparrow$ / FPR@95 $\downarrow$ } \\
\midrule
$\text{ Tiny ImageNet }$ & $\text{ Tiny ObjectNet }$ & 0.51 / 0.96 & 0.82 / 0.51 & 0.79 / 0.63 & 0.75 / 0.74 & 0.70 / 0.68 & 0.72 / 0.75 & \best{0.99} / \best{0.02} & \best{0.99} / \best{0.02} & \secondbest{0.98} / \secondbest{0.12} \\


\bottomrule
\end{tabularx}

==> tables/main_results_acc_at_tnr.tex <==
\setlength{\tabcolsep}{1pt}
\hyphenpenalty10000
\begin{tabularx}{\textwidth}{@{}ll @{}| @{\hskip 0.2cm} XXXX | >{\centering\arraybackslash}XXX @{}} 
\toprule
\makecell[l]{ ID data } & \makecell[l]{ OOD data } & \makecell[l]{ kNN } & \makecell[l]{ Vanilla\\Ensembles } & \makecell[l]{ OE } & \makecell[l]{ Mahal. } & \makecell[c]{ Mahal-T } & \makecell[l]{ MCD } & \makecell[l]{ RETO\\(pretrained) } \\ 
& & \multicolumn{4}{c|}{Inductive} & \multicolumn{3}{c}{Transductive} \\ 
\cmidrule{3-9}
& & \multicolumn{7}{c}{Acc@TNR=95\% $\uparrow$ / TPR@TNR=95\% $\uparrow$ } \\
\midrule
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 2 (A) }$ & 0.32 / 0.11 & \bestnonreto{0.94} / 0.19 & 0.93 / 0.18 & 0.93 / \bestnonreto{0.48} & 0.93 / 0.30 & 0.90 / 0.62 & \bestreto{0.96} / \bestreto{0.93} \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 2 (W) }$ & 0.30 / 0.03 & \bestnonreto{0.98} / 0.06 & 0.97 / 0.05 & 0.93 / \bestnonreto{0.08} & 0.94 / 0.07 & 0.86 / 0.06 & \bestreto{0.96} / \bestreto{0.53} \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 5 (A) }$ & 0.31 / 0.17 & 0.87 / 0.40 & 0.90 / 0.45 & \bestnonreto{0.92} / \bestnonreto{0.76} & 0.91 / 0.56 & 0.91 / 0.89 & \bestreto{0.96} / \bestreto{1.00} \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 5 (W) }$ & 0.33 / 0.05 & \bestnonreto{0.97} / 0.09 & 0.96 / 0.10 & 0.92 / \bestnonreto{0.25} & 0.85 / 0.14 & 0.85 / 0.08 & \bestreto{0.96} / \bestreto{0.96} \\
$\text{ CIFAR100 }$ & $\text{ CIFAR100-C sev 2 (A) }$ & 0.14 / 0.11 & 0.74 / 0.14 & 0.69 / 0.13 & \bestnonreto{0.75} / \bestnonreto{0.43} & 0.71 / 0.15 & 0.51 / 0.42 & \bestreto{0.79} / \bestreto{0.87} \\
$\text{ CIFAR100 }$ & $\text{ CIFAR100-C sev 2 (W) }$ & 0.14 / 0.05 & \bestnonreto{0.83} / 0.06 & 0.78 / 0.06 & 0.78 / \bestnonreto{0.08} & 0.78 / 0.07 & 0.51 / 0.05 & \bestreto{0.80} / \bestreto{0.30} \\
$\text{ CIFAR100 }$ & $\text{ CIFAR100-C sev 5 (A) }$ & 0.14 / 0.17 & 0.64 / 0.22 & 0.60 / 0.24 & \bestnonreto{0.74} / \bestnonreto{0.68} & 0.70 / 0.50 & 0.55 / 0.78 & \bestreto{0.79} / \bestreto{0.99} \\
$\text{ CIFAR100 }$ & $\text{ CIFAR100-C sev 5 (W) }$ & 0.15 / 0.05 & \bestnonreto{0.80} / 0.12 & 0.75 / 0.12 & 0.67 / \bestnonreto{0.16} & 0.64 / 0.10 & 0.46 / 0.09 & \bestreto{0.79} / \bestreto{0.86} \\

\midrule
\multicolumn{2}{c  @{\hskip 0.2cm}}{Average} & 0.23 / 0.14 & 0.80 / 0.24 & 0.78 / 0.25 & \bestnonreto{0.83} / \bestnonreto{0.59} & 0.81 / 0.38 & 0.72 / 0.68 & \bestreto{0.88} / \bestreto{0.95} \\

\bottomrule
\end{tabularx}

==> tables/old_different_ensemble_size_results.tex <==
\hyphenpenalty10000
\begin{tabularx}{\textwidth}{@{}l@{\hskip -0.01cm}l @{} @{\hskip 0.1cm} XX >{\centering\arraybackslash} XX >{\centering\arraybackslash} XX@{}}
\toprule
& & \multicolumn{2}{c}{K=2} & \multicolumn{2}{c}{K=3} & \multicolumn{2}{c}{K=4} \\
\cmidrule(l{2pt}r{2pt}){3-4}
\cmidrule(l{2pt}r{2pt}){5-6}
\cmidrule(l{2pt}r{2pt}){7-8}
\makecell{ID data} & \makecell{OOD data} & \makecell{ERD} & \makecell{ERD++} & \makecell{ERD} & \makecell{ERD++} & \makecell{ERD} & \makecell{ERD++} \\
& & \multicolumn{6}{c}{AUROC $\uparrow$ / TNR@95 $\uparrow$ } \\
\midrule
$\text{ SVHN }$ & $\text{ CIFAR10 }$ & 0.99 / 0.98 & 0.99 / 0.99 & 0.99 / 0.98 & 1.00 / 0.99 & 0.99 / 0.98 & 1.00 / 0.99 \\
$\text{ CIFAR10 }$ & $\text{ SVHN }$ & 1.00 / 1.00 & 1.00 / 1.00 & 1.00 / 1.00 & 1.00 / 1.00 & 1.00 / 1.00 & 1.00 / 1.00 \\
$\text{ CIFAR100 }$ & $\text{ SVHN }$ & 1.00 / 1.00 & 1.00 / 1.00 & 1.00 / 1.00 & 1.00 / 1.00 & 1.00 / 1.00 & 1.00 / 1.00 \\
$\text{ SVHN[0:4] }$ & $\text{ SVHN[5:9] }$ & 0.95 / 0.69 & 0.94 / 0.68 & 0.95 / 0.73 & 0.95 / 0.75 & 0.96 / 0.76 & 0.96 / 0.77 \\
$\text{ CIFAR10[0:4] }$ & $\text{ CIFAR10[5:9] }$ & 0.89 / 0.55 & 0.92 / 0.58 & 0.89 / 0.57 & 0.94 / 0.70 & 0.90 / 0.57 & 0.95 / 0.73 \\
$\text{ CIFAR100[0:49] }$ & $\text{ CIFAR100[50:99] }$ & 0.81 / 0.40 & 0.82 / 0.43 & 0.81 / 0.41 & 0.84 / 0.44 & 0.81 / 0.41 & 0.84 / 0.44 \\


\midrule
\multicolumn{2}{c}{Average} & 0.94 / 0.77 & 0.95 / 0.78 & 0.94 / 0.78 & 0.95 / 0.81 & 0.94 / 0.79 & 0.96 / 0.82 \\

\bottomrule
\end{tabularx}

==> tables/vgg_results.tex <==
\setlength{\tabcolsep}{1pt}
\hyphenpenalty10000
\begin{tabularx}{\textwidth}{@{}ll @{}| @{\hskip 0.2cm} X X X X X X X X X  @{}}
\toprule
\makecell[l]{ ID data } & \makecell[l]{ OOD data } & \makecell[l]{ kNN } & \makecell[l]{ Vanilla\\Ensembles } & \makecell[l]{ DPN } & \makecell[l]{ OE } & \makecell[l]{ Mahal. } & \makecell[l]{ MCD } & \makecell[l]{ Mahal-U } & \makecell[l]{ $\method$ } & \makecell[l]{ $\method$++ } \\
& & \multicolumn{9}{c}{AUROC $\uparrow$ / TNR@95 $\uparrow$} \\
\midrule
$\text{ SVHN }$ & $\text{ CIFAR10 }$ & 0.92 / 0.68 & 0.97 / 0.88 & \bestnonreto{1.00} / \bestnonreto{1.00} & \bestnonreto{1.00} / \bestnonreto{1.00} & 0.99 / 0.98 & 0.97 / 0.85 & 0.99 / 0.95 & \bestreto{0.99} / 0.94 & \bestreto{0.99} / \bestreto{0.98} \\
$\text{ CIFAR10 }$ & $\text{ SVHN }$ & 0.81 / 0.26 & 0.88 / 0.69 & 0.95 / 0.85 & 0.97 / 0.89 & 0.99 / 0.96 & \bestnonreto{1.00} / \bestnonreto{0.98} & 0.99 / 0.96 & \bestreto{1.00} / \bestreto{1.00} & \bestreto{1.00} / \bestreto{1.00} \\
$\text{ SVHN[0:4] }$ & $\text{ SVHN[5:9] }$ & 0.54 / 0.08 & 0.89 / 0.60 & 0.87 / 0.19 & 0.85 / 0.52 & \bestnonreto{0.92} / \bestnonreto{0.71} & 0.91 / 0.51 & 0.91 / 0.63 & 0.93 / 0.63 & \bestreto{0.94} / \bestreto{0.66} \\
$\text{ CIFAR10[0:4] }$ & $\text{ CIFAR10[5:9] }$ & 0.59 / 0.14 & 0.74 / 0.29 & \bestnonreto{0.82} / 0.32 & \bestnonreto{0.82} / \bestnonreto{0.41} & 0.79 / 0.27 & 0.69 / 0.25 & 0.64 / 0.13 & 0.91 / 0.63 & \bestreto{0.95} / \bestreto{0.74} \\

\midrule
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 2 (A) }$ & 0.59 / 0.16 & 0.66 / 0.17 & 0.73 / 0.31 & 0.70 / 0.20 & \bestnonreto{0.84} / \bestnonreto{0.53} & 0.82 / 0.50 & 0.75 / 0.38 & 0.94 / 0.79 & \bestreto{0.98} / \bestreto{0.93} \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 2 (W) }$ & 0.50 / \bestnonreto{0.08} & 0.51 / 0.05 & 0.47 / 0.03 & 0.52 / 0.06 & \bestnonreto{0.58} / \bestnonreto{0.08} & 0.52 / 0.06 & 0.55 / 0.07 & 0.68 / 0.19 & \bestreto{0.77} / \bestreto{0.33} \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 5 (A) }$ & 0.67 / 0.28 & 0.80 / 0.41 & 0.89 / 0.60 & 0.86 / 0.54 & 0.94 / 0.80 & \bestnonreto{0.95} / \bestnonreto{0.84} & 0.88 / 0.63 & 0.99 / 0.96 & \bestreto{1.00} / \bestreto{1.00} \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 5 (W) }$ & 0.51 / 0.06 & 0.58 / 0.10 & 0.72 / 0.10 & 0.63 / 0.11 & \bestnonreto{0.78} / \bestnonreto{0.27} & 0.60 / 0.08 & 0.68 / 0.12 & 0.95 / 0.72 & \bestreto{0.99} / \bestreto{0.99} \\

\midrule
\multicolumn{2}{c | @{\hskip 0.2cm}}{Average} & 0.64 / 0.22 & 0.75 / 0.40 & 0.81 / 0.43 & 0.79 / 0.47 & \bestnonreto{0.85} / \bestnonreto{0.57} & 0.81 / 0.51 & 0.80 / 0.48 & 0.92 / 0.73 & \bestreto{0.95} / \bestreto{0.83} \\

\bottomrule
\end{tabularx}

==> tables/wrn_results.tex <==
\setlength{\tabcolsep}{1pt}
\hyphenpenalty10000
\begin{tabularx}{\textwidth}{@{}ll @{}| @{\hskip 0.2cm} X X X X X X X X X  @{}}
\toprule
\makecell[l]{ ID data } & \makecell[l]{ OOD data } & \makecell[l]{ kNN } & \makecell[l]{ Vanilla\\Ensembles } & \makecell[l]{ DPN } & \makecell[l]{ OE } & \makecell[l]{ Mahal. } & \makecell[l]{ MCD } & \makecell[l]{ Mahal-U } & \makecell[l]{ $\method$ } & \makecell[l]{ $\method$++ } \\
& & \multicolumn{9}{c}{AUROC $\uparrow$ / TNR@95 $\uparrow$} \\
\midrule
$\text{ SVHN }$ & $\text{ CIFAR10 }$ & 0.92 / 0.68 & 0.96 / 0.86 & \bestnonreto{1.00} / \bestnonreto{1.00} & \bestnonreto{1.00} / \bestnonreto{1.00} & 0.99 / 0.98 & 0.97 / 0.85 & 0.99 / 0.95 & \bestreto{1.00} / \bestreto{0.99} & 0.99 / 0.96 \\
$\text{ CIFAR10 }$ & $\text{ SVHN }$ & 0.81 / 0.26 & 0.94 / 0.81 & 0.95 / 0.85 & 0.97 / 0.89 & 0.99 / 0.96 & \bestnonreto{1.00} / \bestnonreto{0.98} & 0.99 / 0.96 & \bestreto{1.00} / \bestreto{1.00} & \bestreto{1.00} / \bestreto{1.00} \\
$\text{ SVHN[0:4] }$ & $\text{ SVHN[5:9] }$ & 0.54 / 0.08 & 0.91 / 0.62 & 0.87 / 0.19 & 0.85 / 0.52 & \bestnonreto{0.92} / \bestnonreto{0.71} & 0.91 / 0.51 & 0.91 / 0.63 & \bestreto{0.96} / \bestreto{0.78} & 0.94 / 0.71 \\
$\text{ CIFAR10[0:4] }$ & $\text{ CIFAR10[5:9] }$ & 0.59 / 0.14 & 0.80 / 0.35 & \bestnonreto{0.82} / 0.32 & \bestnonreto{0.82} / \bestnonreto{0.41} & 0.79 / 0.27 & 0.69 / 0.25 & 0.64 / 0.13 & 0.94 / 0.71 & \bestreto{0.96} / \bestreto{0.80} \\

\midrule
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 2 (A) }$ & 0.59 / 0.16 & 0.69 / 0.18 & 0.73 / 0.31 & 0.70 / 0.20 & \bestnonreto{0.84} / \bestnonreto{0.53} & 0.82 / 0.50 & 0.75 / 0.38 & \bestreto{0.98} / 0.90 & \bestreto{0.98} / \bestreto{0.92} \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 2 (W) }$ & 0.50 / \bestnonreto{0.08} & 0.51 / 0.05 & 0.47 / 0.03 & 0.52 / 0.06 & \bestnonreto{0.58} / \bestnonreto{0.08} & 0.52 / 0.06 & 0.55 / 0.07 & 0.84 / 0.35 & \bestreto{0.90} / \bestreto{0.57} \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 5 (A) }$ & 0.67 / 0.28 & 0.84 / 0.47 & 0.89 / 0.60 & 0.86 / 0.54 & 0.94 / 0.80 & \bestnonreto{0.95} / \bestnonreto{0.84} & 0.88 / 0.63 & \bestreto{1.00} / \bestreto{1.00} & \bestreto{1.00} / 0.99 \\
$\text{ CIFAR10 }$ & $\text{ CIFAR10-C sev 5 (W) }$ & 0.51 / 0.06 & 0.59 / 0.09 & 0.72 / 0.10 & 0.63 / 0.11 & \bestnonreto{0.78} / \bestnonreto{0.27} & 0.60 / 0.08 & 0.68 / 0.12 & 0.99 / 0.97 & \bestreto{1.00} / \bestreto{0.98} \\

\midrule
\multicolumn{2}{c | @{\hskip 0.2cm}}{Average} & 0.64 / 0.22 & 0.78 / 0.43 & 0.81 / 0.43 & 0.79 / 0.47 & \bestnonreto{0.85} / \bestnonreto{0.57} & 0.81 / 0.51 & 0.80 / 0.48 & 0.96 / 0.84 & \bestreto{0.97} / \bestreto{0.87} \\

\bottomrule
\end{tabularx}
